Bayesian semi-parametric inference for clustered recurrent events with zero-inflation and a terminal event/4163305

Recurrent event data are common in clinical studies when participants are followed longitudinally, and are often subject to a terminal event. With the increasing popularity of large pragmatic trials with a heterogeneous source population, participants are often nested in clinics and can be either susceptible or structurally unsusceptible to the recurrent process. These complications require new modeling strategies to accommodate potential zero-event inflation as well as hierarchical data structures in both the terminal and non-terminal event processes. In this paper, we develop a Bayesian semi-parametric model to jointly characterize the zero-inflated recurrent event process and the terminal event process. We use a point mass mixture of non-homogeneous Poisson processes to describe the recurrent intensity and introduce shared random effects from different sources to bridge the non-terminal and terminal event processes. To achieve robustness, we consider nonparametric Dirichlet processes to model the residual of the accelerated failure time model for the survival process as well as the cluster-specific frailty distribution, and develop a Markov Chain Monte Carlo algorithm for posterior inference. We demonstrate the superiority of our proposed model compared with competing models via simulations and apply our method to a pragmatic cluster randomized trial for fall injury prevention among the elderly.

==> latexmkrc <==
# HACK: this width seems to change with every compile, so
# latexmk runs latex too many times; ignore it
$hash_calc_ignore_pattern{'aux'} = 'statsocwidth';

# All the other default settings on Overleaf
# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
